Survive the Schema Changes: Integration of Unmanaged Data Using Deep Learning

Data is the king in the age of AI. However data integration is often a laborious task that is hard to automate. Schema change is one significant obstacle to the automation of the end-to-end data integration process. Although there exist mechanisms such as query discovery and schema modification language to handle the problem, these approaches can only work with the assumption that the schema is maintained by a database. However, we observe diversified schema changes in heterogeneous data and open data, most of which has no schema defined. In this work, we propose to use deep learning to automatically deal with schema changes through a super cell representation and automatic injection of perturbations to the training data to make the model robust to schema changes. Our experimental results demonstrate that our proposed approach is effective for two real-world data integration scenarios: coronavirus data integration, and machine log integration.

==> experiments.tex <==
\section{Experimental Results}
\label{sec:experiments}
\subsection{Environment Setup}
We implement the deep learning approach using TensorFlow version $1.14$, CUDA version $10$ and python, and the baseline approach also in python using pandas APIs. We deploy the system in a desktop installing Intel i$7$ CPU, $32$ GB memory, and Nvidia RTX $2070$ Super GPU with $8$ GB Memory.
 

We mainly evaluate our system in two COVID-$19$ data integration scenarios that are close to the example in Sec.~\ref{sec:problem}. In the first scenario, we predict COVID-$19$ death using daily and regional information regarding number of confirmed cases and a mobility factor.  From a set of raw data sources, we need create a time-series $2$-dimensional array, where each row represents data for a state/province on a specific date, and each column represents date, state, country, the number of confirmed cases, and the value of mobility factor, which can be used as inputs to various curve-fitting techniques~\cite{death-prediction-cdc, covid19-models} for COVID-$19$ death prediction. In the second scenario, we use regional information including total population, male population, female population, number of hospitals, number of ICUs and so on for COVID-$19$ death prediction. 

We assume the user specifies/recommends a small set of initial data sources. For the first scenario, the user specifies the John Hopkins University's COVID-$19$ github repository~\cite{covid19-jhu} and Google mobility data~\cite{google-mobility}. For the second scenario, a dataset from Kaiser Health News~\cite{icu-beds} and a dataset from Harvard dataverse COVID-$19$ repository~\cite{covid19-harvard} are used. In the first scenario, both of the two source datasets are updated at daily basis and observed with frequent schema changes. The statistics about the above source tables are illustrated in Tab.~\ref{tab:table-statistics}.

For both models, we use $256$ neurons for the first layer and the third layer respectively. For the last layer, we use $512$ neurons for LSTM, and for CNN, we use three conv$2$D and pooling layers, each of which uses $100$ $3\times3$, $4\times4$, and $5\times5$ filters respectively and $1$ stride. We use learning rate of $0.001$ and batch size of $256$.

\begin{table}[h]
\centering
\scriptsize
\caption{\label{tab:table-statistics} Statistics of Relevant Data Sources.}
\begin{tabular}{|c|r|r|} \hline
&numRows&numCols\\\hline \hline
JHU-COVID-$19$&$310$&$66$\\ \hline
Google-Mobility&$477322$&$11$\\ \hline
KHN-COVID-$19$&$3142$&$11$\\ \hline
Harvard-COVID-$19$&$3143$&$459$\\ \hline
\end{tabular}
\end{table}

We then evaluate the accuracy and the end-to-end latency of the trained models for synthetic data with schema changes applied (we do not consider column expansion and contraction in preliminary experiments) and data that is irrelevant with the target tables that are synthesized from real-world COVID-$19$ data as illustrated in Tab.~\ref{tab:all-statistics}. The accuracy of the data integration model is defined as the ratio of the number of correctly classified data cells to the total tested classified data cells.

\begin{table}[h]
\centering
\scriptsize
\caption{\label{tab:all-statistics} Statistics of open CSV COVID-19 data that we've collected in the data repository.}
\begin{tabular}{|c|c|c|} \hline
numFiles&avgNumAttributes (Width) &avgNumRows (Depth)\\\hline \hline
$2306$&$65$&$3422$\\ \hline
\end{tabular}
\end{table}

\vspace{-20pt}

\subsection{Testing Accuracy Analysis}
The model testing accuracy for the first scenario with time series and regional information is illustrated in Tab.~\ref{tab:accuracy}. In total, the training dataset includes $28751$ automatically labeled training samples. We observe that using CNN achieves significantly higher accuracy in various testing cases, particularly for testing with partially irrelevant data cells. This is mainly because CNN considers the locality of features while sequence is less important for this case.

\begin{table}[h]
\centering
\scriptsize
\caption{\label{tab:accuracy} Testing Accuracy Comparison.}
\begin{tabular}{|l|c|c|} \hline
Testing Cases&LSTM&CNN\\\hline \hline
Relevant data with no schema changes&$98.76\%$&$99.29\%$\\ \hline
Relevant data with schema changes&$98.13\%$&$99.92\%$\\ \hline
Totally irrelevant data&$99.96\%$&$99.04\%$\\ \hline
Partially irrelevant data&$67.16\%$&$98.41\%$\\ \hline
\end{tabular}
\end{table}

For the second scenario with only regional information, we only try the LSTM model and it can achieve $100\%$ accuracy for relevant data with no schema changes, and we didn't test with other cases, which we will leave to future works.

We see an obvious advantage of our proposed deep learning approach compared to the baseline approach. For example, the baseline approach cannot handle the first scenario as illustrated in Fig.~\ref{fig:schema-example} where the time-series dimension is pivoted and can be hardly mapped to any column in the target table. However, in the second scenario, the baseline approach can correctly identify all related attributes and map attributes in the source datasets to the target table. 

\subsection{Latency Analysis}
We also test and compare the end-to-end latency including training and testing of the deep learning approach to the baseline approach. The results are illustrated in Tab.~\ref{tab:latency}. 

\begin{table*}[h]
\centering
\scriptsize
\caption{\label{tab:latency} Latency break-down and comparison (Unit: second).}
\begin{tabular}{|l|r|l|} \hline
&Latency&Measurement details\\\hline \hline
Data-decomposition-scenario1&$7.47$&JHU and Google mobility datasets\\ \hline
Traing-latency-LSTM-scenario1&$11.37$&for $28751$ training samples\\ \hline
Testing-latency-LSTM-scenario1&$6.3$&for $30000$ testing samples\\ \hline
Traing-latency-CNN-scenario1&$7.52$&for $28751$ training samples\\ \hline
Testing-latency-CNN-scenario1&$3.66$&for $30000$ testing samples\\ \hline
Data-decomposition-scenario2&$8.14$&Harvard and KHN datasets\\ \hline
Training-latency-LSTM-scenario2&$6.93$&for $5000$ training samples\\ \hline
Testing-latency-LSTM-scenario2&$0.17$&for $1000$ testing samples\\ \hline
Baseline-approach-creating-LSH-scenario2&$14.65$&for $11$ columns in KHN data and $459$ columns in Harvard data\\ \hline
Baseline-approach-matching-LSH-scenario2&$23.21$&for $11$ columns in KHN data and $459$ columns in Harvard data\\ \hline
Baseline-approach-join-scenario2&$0.04$&using pd.DataFrame.merge()\\ \hline
\end{tabular}
\end{table*}

\vspace{-10pt}

\subsection{Storage Overhead Analysis}
We find that the deep learning approach has an obvious benefit in saving storage overhead compared to the baseline approach. Each LSTM model has $1000$ parameters in total, which is $16$ KB in size, and the CNN model has $5500$ parameters, which is $88$ KB. However, for the baseline approach, we store $512$ MinHash LSH signatures~\cite{indyk1998approximate} for each column and each signature has $4$ bytes, so it takes $154$ KB for the JHU COVID-$19$ dataset and the Google mobility dataset in the first scenario, and $940$ KB for the Harvard and KHN COVID-$19$ datasets in the second scenario. If consider all $2306$ CSV files (Tab~\ref{tab:all-statistics}, it requires $300$ MB of storage overhead in total, while the deep learning approach only needs to store the model that is smaller than $100$ KB.



==> intro.tex <==
\section{Introduction}

Data scientists spent $80$-$90$\% efforts in the data integration and wrangling process~\cite{abadi2020seattle, stonebraker2018data, thirumuruganathan2018data}. Although there exist a lot of works trying to facilitate or accelerate this process, including the automation in entity matching~\cite{mudgal2018deep, meduri2020comprehensive, kasai2019low, konda2016magellan,thirumuruganathan2018reuse, zhao2019auto, ebraheem2017deeper}, schema discovery and matching~\cite{fernandez2018aurum,fernandez2018seeping,zhu2016lsh,zhu2019josie,nargesian2018table,nargesian2020organizing}, and so on, however there is still no end-to-end automatic data integration pipeline that directly drives features from raw data without much human intervention~\cite{abadi2020seattle, stonebraker2018data, thirumuruganathan2018data}. 

Given the vast variety of data integration requirements of different machine learning applications, it is challenging to provide one end-to-end system for all heterogeneous data integration problems. While domain-specific systems are more reasonable to automate various data integration problems, they suffer from the fast evolution of data schemas, which may easily break an automated pipeline. Taking the COVID-$19$ data repository~\cite{covid19-jhu} maintained by the Johns Hopkins University for example, not only the data contents are updated at an daily basis, the data schema also changes frequently. For example, by checking the github commit history, we find their schema changed for five times in March $2020$~\cite{covid19-jhu}. Typical schema changes include:

\noindent
1. \textbf{Dimension pivoting}. As illustrated in Fig.~\ref{fig:schema-example}), two time-series tables for COVID-19 death cases and confirmed cases respectively can pivoted into a set of new tables with each table describing both death and confirmed cases for a specific date. We find such schema change not only in the JHU COVID-$19$ repository, but also in many other data sources such as the weather datasets in the National Climatic Data Center's data repository~\cite{}.

\noindent
2. \textbf{Attribute name changes}. For example, we find a number of such schema in the JHU COVID-$19$ repository, including: "Province/State" $\rightarrow$ "Province\_State", "Country/Region" $\rightarrow$ "Country\_Region", "Longitude" $\rightarrow$ "Long\_", "Latitude" $\rightarrow$ "Lat", and so on.

\noindent
3. \textbf{Attribute addition/removal}. For example, in the JHU COVID-$19$ repository, the initial data schema only had seven attributes, but now it has fourteen attributes.

\noindent
4. \textbf{Key expansion/contraction}. As illustrated in Fig.~\ref{fig:prediction}, we find in the JHU COVID-$19$ repository that the initial table only includes the state-level information so that the initial primary key of each table consists of only two attributes: "Province/State" and "Country/Region". But later the table is expanded to include the county information, so the primary key has three attributes: "Province/State", "Country/Region", and "Admin2" (i.e. county name). Similarly, key contraction may also happen. For example, for US COVID-19 information, a single FIPS ID attribute can replace the above three attributes to serve as a primary key.

Consider integrating such fast evolving data sources for a data science application, because the data content updates fast, the application need to periodically run the data integration process to get up-to-date integrated data. However, because the schema also evolves, it may happen that previous versions of data integration programs cannot work correctly anymore. It will incur huge burden on the data scientist if s/he needs to tweak the integration code every time. Such situation is ubiquitous in analytics regarding pandemics such as COVID-19 or sensor data integration scenarios where heterogeneous devices will use different data schemas. {\color{red}{TODO}}

In this paper, we focus on automating the process of driving features from such fast evolving raw data sources.  We argue that if the integration outcome data required by an application is relatively stable compared to the varieties and dynamics in both data sources' schemas and contents, a deep learning approach can well automate the periodical data integration processes without human intervention. A deep learning approach can also achieve better accuracy, latency and significantly lower storage overhead in the end-to-end process than a baseline data integration approach, which first discovers related data using locality sensitive hashing (LSH)~\cite{gionis1999similarity, indyk1998approximate} and then integrates data through fuzzy join or union operations. 



We observe that while a dataset may be represented in different ways at different time points, we can always map these different representations into an abstracted key-value based data model. Then it is feasible to learn a mapping between the abstract data model and the user desired outcome table. As illustrated in Fig.~\ref{fig:schema-example}, despite of various schema changes, the mapping from the data model to the user desired integrated table is relatively constant, and can be learned through deep learning.


\begin{figure*} 
\centering
   \includegraphics[width=5in]{schema-example.pdf}
\caption{\label{fig:schema-example}
Mappings among source data (with dimension-pivoting applied), abstract data model and user-desired output table.}
\vspace{-10pt}
\end{figure*}


Based on above observation, we formalize the data model as a list of quadruples in the form of (\texttt{key\_array}, \texttt{key\_type\_array}, \texttt{value}, \texttt{value\_type}). We then train a deep learning model that learns the mapping between the abstract data model and the user-desired table. The trained model can be used to transform raw data collected from fast-evolving sources into user-desired tables, of which the process is adaptive to schema evolution. First, each raw dataset, is decomposed into a stream of quadruples based on the abstract data model. Second, each quadruples serves as features, for which the model should predict its position in the outcome table (i.e. attribute name and row key values), and an aggregation mode that specifies how this value should be aggregated with other values mapped to the same position in this table. We support aggregation modes like \texttt{+}, \texttt{max}, \texttt{min}, \texttt{replace}, \texttt{concat}, \texttt{discard}, and so on. Based on this idea, we design an end-to-end system that automates the data integration process. The system provides interfaces for (1) registering new data sources; (2) issuing a data integration request by specifying the schema of the desired outcome table\eat{, including a list of column names and a list of acceptable row-keys (or rules for populating row-keys)}; (3) training and managing models. We compare two types of model architectures in this work. In both types, the first layer is a word embedding layer, and the 
last layer is a fully connected layer. The difference is that in the first type, we use three Conv$2$D and pooling layers in middle, but in the second type, we use a bi-LSTM layer in middle. We find in our preliminary results that the CNN-based model can achieve better accuracy than the LSTM-based model.

\eat{
Each time the user needs to collect a set of feature vectors for his/her data science application, instead of manually exploring and integrating all available data sources, and identifying and handling the schema changes, they can use our system to drive features directly from the raw, heterogeneous, and fast-evolving data sources. More importantly, the pre-trained data integration models can be easily shared across a group of users in our system, by associating each model with the schema and example values of the expected outcome table. Then when a user submits a data integration request by specifying a small example of his/her expected outcome table, our system will automatically decide whether there exists a pre-trained data integration model that can be reused for the new data integration task by creating and matching a high-dimensional signature over these expected tables. }

Through experiments, we also observe that compared to a baseline data integration approach that requires to store LSH signatures for each column, our proposed approach incurs merely constant storage overheads, which may save significant amount of storage space, particularly for wide tables. In addition, for integrating wide and/or sparse datasets, we also observe a computational advantage in the deep learning approach. Moreover, our approach can seamlessly handle heterogeneous data sources and schema evolution without any additional LSH re-computation and storage overheads.

Usually a major concern over a deep learning approach is that the training process may take a lot of domain experts' efforts in labeling data. However, we argue that in our targeting scenario, the data labeling process can be largely automated if human experts are able to find a bootstrapping high-level mapping between the initial data source and the target outcome table. Then, the labeling can be fully automated and even the schema changes can be automatically injected to enhance the training data. Once the models are trained,  they can handle most of schema evolution cases without any human intervention. 

We summarize our key contributions as following:
\begin{itemize}
    \item We propose and formalize a deep-learning approach to address the problem of end-to-end automatic data integration of the fast-evolving CSV files.
    \item We share experiences of the system design and model training.
    \item We design and implement a prototype of the system and give a preliminary evaluation with detailed analysis for the proposed approach. 
\end{itemize}

In the rest of the work, we will first introduce related works in Sec.~\ref{sec:survey}. Then we will formalize the problem in Sec.~\ref{sec:problem}. Following that, we will propose a baseline approach and a deep learning approach in Sec.~\ref{sec:solution}. Finally, we will present our preliminary experimental results in Sec.~\ref{sec:experiments} and conclude the paper.


==> new_intro-punched.tex <==
\section{Introduction}
In Big Data era, when the data is not a precious resource, error in data is more tolerable in analytics than ever~\cite{}. That is, given the large volume of input data, if most of the data is correct, the accuracy of the upper-layer analytics applications will be hardly impaired by a few errors~\cite{}. This observation motivates us to use a deep learning approach, which is sometimes more economic as we will elaborate later, to replace a few expensive database operations such as equi-join and similarity join (or fuzzy-join). 

Equi-join and fuzzy join are both common operations widely used in data integration and analytics applications. As illustrated in Fig.~\ref{}, equi-join is to join pairs of tuples that have the same value(s) on the specified attribute(s); and fuzzy-join is to join pairs of tuples that have similar value(s) on the specified attribute(s). It is well-known that applying these two operations to large datasets are usually expensive as the amount of intermediate pairs of tuples could grow exponentially. There are numerous optimization techniques proposed to optimize their efficiency~\cite{} of equi-join. Most famously, pre-partitioning of the input datasets for equi-join~\cite{} can transform a distributed join into local joins and thus it can get rid of the most expensive distributed shuffling operation. However, the amount of intermediate data at each local node still could be explosive. Another popular approach widely applied to query optimization is to push down the join filtering and projection predicates to reduce the volume of intermediate data. In addition, approximated join has also been widely explored to estimate the join results based on synopsis of the input datasets~\cite{}. For fuzzy join, locality sensitive hashing is usually utilized to reduce the problem into an equi-join problem by associating each tuple with multiple LSH signatures~\cite{}. However as said the equi-join is still among the most expensive operations. 

This work argues for a unified deep learning approach to improve the performance of and alleviate the memory overhead required for both of the equi-join and similarity join operations. As illustrated in Fig.~\ref{}, if the schema and keys of the output table is known, then the join can be seen as a function that maps each cell to a position in the output table, which is indexed by the attribute name and row key values. In our work, we attempt to demonstrate that this relationship can be learned using neural network models. In addition, we further demonstrate that the size of the model that meets an acceptable accuracy requirement, is usually significantly smaller than the total size of the intermediate data in a database join, and thus can handle many large-scale join operations that will fail in a relational database due to the lack in memory resources.

However, there are no gain without pains. Major challenges facing the learning-based join process are: First, how to obtain the keys in the output table? Second, how to select/implement the model architecture, text representation and embedding, and label space representation to improve the accuracy? Third, how to reduce the overheads associated with the training process?  We describe the approaches we used to address these problems as following:

\noindent
\textbf{Output Key Enumeration.} We find that the keys on the output of a join operation can often be derived based on relational model and functional dependency.

For example, if A joins B on A's foreign key to B, $1$-$1$ or $N$-$1$ relationship is thus maintained (i.e., for each tuple in A, there is one and only one tuple in B that can match A, and it is possible that multiple tuples in A correspond to the same tuple in B.). In this case, we call A as the \textit{dominant} table. Then the output's key is A's key, and the set of key values of the output is a subset of the set of key values of A. \textit{Example: Orders table joins Customers table on CustomerID.} 

Another example is that if A and B share the same key and A joins B on the shared key, $1$-$1$ relationship is maintained in the join (i.e., for each tuple in A there is one tuple in B that can match A, and vice versa.). In this case, the table A or B that has larger size of keys is the dominant table. Then the output's key is A's key (or B's key), and the set of key values of the output is the intersection of the set of key values of A and the set of key values of B. \textit{Example: population by region joins coronavirus cases by region.}

In addition, there is a rare situation where A joins B on a set of shared non-key attributes. In this case, an $N$-$M$ relationship maybe observed during the matching process (i.e., each tuple in A matches $N$ tuples in B, and for each tuple in B there are $M$ tuples in A that are matched.).  Then the output's key is the combination of  A's key and B's key, and the set of key values of the join output is a subset of the set of values of the cartesian product of the set of A's key values and B's key values. \textit{Example: dblp publication dataset joins Google news dataset on the year information.}

We find in TPC-H and TPC-DS benchmarks, most of the queries are following the first two cases, for which the enumeration of keys for the join output is easy and efficient, with the memory requirements equivalent to the size of the set of keys of the dominant table. In this work, we focus on these two cases. In addition, we introduce super key in the join output, which can be obtained upon the afore-mentioned key derivation process to provide more information to the learning process and thus achieve better accuracy. 

\noindent
\textbf{Model and Representation.} First all text attribute names or values need to be converted to a vector through an embedding so that the vectors for more related texts are closer in the embedding space. Text embedding is a hot research area, and there are a lot of pre-trained embeddings available for use, which are trained in public corpus like Wikipedia, Google News, Common Crawl and so on. We call these embeddings as distributed embedding. In contrary, we can also create local corpus on each table using a random walk approach~\cite{}, and extract local embeddings from such corpus. Besides there are also character-based embedding like FastText and word-based embedding like word2Vec. We find that character-based embedding and local embedding can outperform other alternatives in most cases. In addition, we extend existing local embedding approach to more efficiently handle a database of tables utilizing the functional dependency.

Second, we discuss about the label representation. If a two-way join is under the $1$-$1$ mapping, a cell in any table should be mapped to at most one position in the output table. However, if it is under the $N$-$1$ mapping, a cell may be placed in more than one positions. So we model the label space as a probability distribution over all attribute names and row super keys, then we sample one attribute name and one or multiple super keys. We can finally determine the position(s) of an input cell by combining the attribute with the row keys.

Third, given the input represented as a sequence of separated embedding vectors, and label represented as probability distribution over a set of attributes and row keys, a broad class of models can fit in the niche. We mainly experiment with Bi-LSTM, LSTM and CNN.




\noindent
\textbf{Transferable Training Process.}
Training is an expensive process and it is expected that one training will benefit a large number of testing cases, so that the training overhead can be amortized to the testing phase. In this work, we mainly consider and investigate three training paradigms: 

The first paradigm is to train on a subset of the datasets to be joined, which assumes that the relationships learnt on the subset can be extended to the whole datasets. 

The second is to train on the wholeset of the datasets, and then the trained model is used like a compressed view, and users can easily use the model to map the input datasets to various subsets of join output with attributes projected and rows filtered in different ways.

The third one is to train the model through transfer learning. If two different join problems involve similar vocabularies, the knowledge learned in the source problem maybe transferable to the target problem. We designed a metric based on JS-divergence to select related source model for a given target problem.




While deep learning and/or reinforcement learning are widely applied to the cardinality/selectivity analysis or execution plan selection, of the join operations, we are the first to directly use deep learning to perform a join operation. The main contributions of our work include:




==> new_intro.tex <==
\section{Introduction}
It was reported in 2018 that data scientists spent $80$-$90$\% efforts in the data integration and wrangling process~\cite{abadi2020seattle, stonebraker2018data, thirumuruganathan2018data}. In this work, we identify that in the era of Big Data and Internet of Things, the schema change in open data, is one of the main factors leading to the tremendous overhead involved in data integration. Schema changes include two types: schema evolution and heterogeneous schema. Schema evolution is ubiquitous in agile development environment and data migration due to schema evolution accounted for $31$\% of IT project budgets in 2011~\cite{howard2011data}; and heterogeneous schema is caused by the lack of standards in many domains such as sensor data and spatial-temporal data, for example the same type of temperature sensor produced by different manufacturers may use different formats to report data. 

Considering a data processing pipeline that automatically and continuously integrates data sources through join or union-alike operations coded up in python to create training data or testing features for artificial intelligence applications, frequent schema changes in one or more of the data sources could interrupt the pipeline and usually require human interventions to fix the problem by either changing the code or migrating all data sources that contain similar data to one unified format. Such interruptions not only incurs human development costs, but also limit the deployment and adoption of models and delay the decision process. However, there is still no effective solution to alleviate this problem.

\eat{
Let's use two real-world examples to illustrate the problem:

\noindent
\textbf{1. Schema evolution in COVID-19 data integration.} It's well known that schema evolution is ubiquitous in enterprise database~\cite{} and website database such as the wikipedia database~\cite{}.It also widely exists in open data.  
\noindent
\textbf{2. Diversified schema in sensor data integration.} A hospital purchases medical sensor devices from more than one manufacturers for measuring temperature, pressure, vibration, sound level, light intensity, load or weight, flow rate of gases and liquids, amplitude of magnetic and electronic fields, and concentrations of many substances in gaseous, liquid, or solid form~\cite{campbell2016plea,al2016iot}. These sensors may output data in various formats: binary, JSON, XML, texts. Even if the two sensor devices use the same format, the representation maybe different. Many medical applications require to integrate such multi-channel time-series data from hundreds to thousands of patients to train predictive models. However, because of such diversified formats of sensors, the data integration application developed in one hospital often needs to be changed multiple times when new sensors are added. Also the application cannot be developed once and used in other hospitals. Diversified schema is usually caused by the lack of the standards, which is ubiquitous in other domains such as spatial temporal data, machine log data, social media data, and so on.
}
\eat{
\noindent
\textbf{Motivating Scenario 2. Machine Data Integration.} Suppose a lab administrator developed a python tool to integrate various performance metrics of a cluster of MacOS workstations, such as CPU utilization (user, system, idle, wait), memory utilization (cached, buffered, swap), network utilization (input, output), disk utilization (write, read), and so on. The tool collect these metrics by periodically reading the output of an omnipresent shell tool "top"~\cite{} and then union metrics collected from each machine. Now the lab purchased four Ubuntu Linux servers. However, because the "top" tool's output in Ubuntu is very different with MacOS, the python tool cannot work with these new Linux machines without additional coding efforts. Such problem is prevalent in machine or sensor data integration, where different devices produced by different manufacturers may use different schemas to describe similar information~\cite{}.}


\noindent
\textbf{Prior arts.} Schema evolution in relational databases and NoSQL databases and heterogeneous schema in multi-model databases are both well-established research topics. The fundamental idea of most existing works in this area is to capture the transformation semantics between the old schema and the new schema, so that the legacy queries or applications can be transformed and/or legacy data can be migrated to work with the new schemas. There are two general approaches to capture the transformation semantics: 

\noindent
(1) To search for the queries that can transform the old schema to the new schema~\cite{miller2000schema, hernandez2001clio, popa2002mapping, an2007semantic, fagin2009clio, shen2014discovering}. This is often utilized in relational database.

\noindent
(2) To ask the database administrators (DBAs) or application develops to use a domain-specific language to describe the schema transformation process~\cite{bernstein2007model, herrmann2017living, curino2013automating, moon2009prima, herrmann2015codel, hillenbrand2019migcast, moller2019query, klettkeevolution, moon2010scalable, scherzinger2013managing}, and then an optimal data migration plan can be searched, and the legacy data can be automatically migrated to conform to the new schema. This is often discussed in the context of both relational databases~\cite{bernstein2007model, herrmann2017living, curino2013automating, moon2009prima, herrmann2015codel} and NoSQL databases~\cite{hillenbrand2019migcast, moller2019query, klettkeevolution, moon2010scalable, scherzinger2013managing, storl2018curating}.  


However, these approaches are not applicable to open data, which are publicly available CSV, JSON, HTML, or text files that can be directly downloaded from a url. These are often not managed by any data stores, relational or NoSQL. As a result, it is hard for an open data integration pipeline to track and manage the schema evolution in data sources on behalf of the these sources' owners, who are totally behind the scenes. We can store each copy of downloaded data into relational or NoSQL databases, and use their language to describe observed schema changes. But this process requires significant human efforts, which may amount to the overhead of manually handling the interruptions caused by schema changes. This process will become even more complicated, given that a lot of open data lacks schema, or have diversified schema.

\eat{In addition, the data integration application running on top of these data is often coded up in a high-level language like Python, Java, R, which lacks an intermediate representation like relational algebra that is easy to modify so that old code can be automatically transformed to work with the new schema.} 

\noindent
\textbf{A deep learning approach.} In this work, we argue for a new data integration pipeline that uses deep learning to avoid interruptions caused by the schema changes. In the past few years, deep learning (DL) has become the most popular direction in machine learning and artificial intelligence~\cite{lecun2015deep, schmidhuber2015deep}, and has transformed a lot of research areas, such as image recognition, computer vision, speech recognition, natural language processing, and so on, and in recent, it is applied to database systems and applications to facilitate parameter tuning~\cite{van2017automatic, sullivan2004using, li2019qtune, zhang2019end}, indexing~\cite{kraska2018case, ding2020alex}, partitioning~\cite{DBLP:journals/corr/abs-2006-16529, DBLP:conf/sigmod/HilprechtBR20}, cardinality estimation and query optimization~\cite{kipf2018learned, krishnan2018learning}, and entity matching~\cite{mudgal2018deep, kasai2019low, konda2016magellan,thirumuruganathan2018reuse, zhao2019auto, ebraheem2017deeper}. While predictions based on deep learning cannot guarantee correctness, in Big Data era, errors in data integration are usually tolerable as long as most of the data is correct, which is another motivation for our work. As to our knowledge, we are the first to apply deep learning to learn the process of join/union-like operations with schema changes occurring in the data sources.

Our approach is illustrated in Fig.~\ref{fig:motivation}. Different with existing approaches, our main idea is to formulate a prediction problem that tells the position of each cell, which is the smallest unit of a database table, based on the cell's context and value (See Sec.~\ref{representations}). Cells that have similar mapping patterns can be grouped into a super cell representation to reduce the training and prediction latency. We have achieved promising results on this task by using compact and efficient models based on Long Short Term Memory (LSTM) and Convolutional Neural Network (CNN) for union and $1$-$1$ join. We propose to apply Mask language model based on attention network and transformer to improve the accuracy for more complicated scenarios such as $1$-$N$ join and $N$-$M$ join (See Sec.~\ref{models}). \eat{The target position is indexed by the target cell's local key (e.g. key as a tuple identifier) and remote key (e.g. foreign key in relational database). The source cell's context include information such as the local key, remote key, attribute name, cell value and so on in the source dataset.} 
Most importantly, we propose to leverage our PlinyCompute intermediate representation~\cite{zou2018plinycompute, zou2020lachesis} to automatically translate user's data integration code for a initial set of data sources into code that creates training data for the prediction task. Context that describes a cell, including local key (i.e. tuple/object identifier), remote key (i.e. foreign key), as well as attribute information, is automatically inferred through the translation process and do not rely on any pre-defined schema (See Sec.~\ref{automation}). In addition to that, specially designed perturbations are automatically added to the training data to make the model robust to schema changes (See Sec.~\ref{schemas}).


\eat{
Further more, we propose to: (1) compare different model architectures including CNN, bi-LSTM, and Attention Network to train deep learning models for our formulated prediction problem using AWS SageMaker (See Sec.~\ref{models}); (2) automate the training data generation using a declarative domain specific language (which can be embedded into Turing-complete languages) for application developers to describe the data integration process, so that user only need to specify what to integrate for a initial set of data sources, and training data will be automatically created with schema changes perturbed (See Sec.~\ref{automation}).}

\begin{figure*}
\centering
\subfigure[A human-centered approach]{%
   \label{fig:huamn}
   \includegraphics[width=3.3in]{before.pdf}  
}%
\subfigure[An deep learning approach (our proposal)]{%
  \label{fig:autoamtic}
  \includegraphics[width=3.3in]{after.pdf}
}
\caption{\label{fig:motivation}
Motivation and Overview of Our Proposed Approach.
}
\end{figure*}

\eat{
\noindent
\textbf{Preliminary results.} We find the schema of John Hopkins University (JHU)'s data repository has changed for tens of times in the first four months. We trained a deep learning model based on bi-LSTM using character-based local embedding for integrating data to predict coronavirus outbreak that requires to continuously join the Google mobility data and the JHU's data. The results show that the model can achieve $97.5\%$ accuracy in handling various types of schema changes\eat{including include attribute name changes (e.g., Longitude $\rightarrow$ Long\_), addition and removal of attributes (e.g., from six attributes initially to $15$ attributes), attribute type changes (e.g., date formats), key changes (e.g., from (\underline{country/region}, \underline{province/state}) to (\underline{combined\_key}), (\underline{FIPS}) and  (\underline{country\_region}, \underline{province\_state}, \underline{Admin2})}. We also find the formats of Unix performance monitoring tools like \textit{top} on different versions of operating systems, e.g. Linux, MacOS, Android, are all different. We create a deep learning model based on bi-LSTM to integrate such heterogeneous data captured at different times on different machines, and union these data to a unified format. The accuracy can achieve $91.2\%$. In the mean time, the inference latency is almost similar to an in-database approach. In addition, our approach doesn't require to store large volume of intermediate pairs for a join or cross product, which could save memory while the model size is only a few kilobytes, which is significantly smaller than even the lightest-weight transformer models. }

\noindent
\textbf{Integration with AWS Products.} We plan to use AWS SageMaker for training (with MXNET) and deploying of the models for various data integration tasks. We believe AWS SageMaker and MXNET can tremendously simplify and accelerate the training process. In addition, at the serving time, SageMaker can help detect concept drifting, and adapt models to various edge devices (e.g. gateways, content delivery nework (CDN), etc.) which serve as rendezvous of multiple data streams. The proposed work also has the potential to benefit AWS data integration service such as Glue in the future. 


==> overview.tex <==
\section{Solution}
\label{sec:solution}
In this section, we will first present a baseline approach that applies existing data discovery techniques for a simplified data integration problem and analyze its limitations. Then we will propose an end-to-end deep learning approach as a more general and more automated solution to our targeting data integration problem. 
\subsection{A Baseline Data Integration Approach}
\label{sec:baseline}
We first simplify the problem by assuming that all raw datasets are structured datasets. Then $d_i \in D$ can be represented as a list of columns, denoted as $d_i = \{a_{ik}\} (0 \leq k < p_i)$, where $a_{ik}$ is the $k$-th column in $d_i$. 

For this simplified problem, we can apply existing data discovery techniques~\cite{zhu2019josie, zhu2016lsh} based on LSH to discover the most similar column in the raw data repository to each column specified in the user desired output. First, the algorithm computes locality sensitive hash (LSH) signatures for each column in the source raw datasets and the user-provided example of the target dataset, then it identifies matching columns, and formulates queries over these matching datasets to create the output integrated dataset. 

 First, for each column in the structured raw datasets $a_{ik} \in d_i$, we create $L$ LSH signatures using a family of $L$ hash functions, denoted as $H^s_{ik} = (h^s_{ik1}, ..., h^s_{ikL})$ and insert each signature into its corresponding hashmap. 

Then, for each column $a_k' \in A^t (0 \leq k' < p)$ in the example of the expected outcome table $V^{A^t \times R^t}$ ) as specified by the user in its data integration request), we also create $L$ LSH signatures, denoted as $H^t_{k'} = (h^t_{k'1}, ..., h^t_{k'L})$. 

After that, every pair of $\langle H^s_{ik}, H^t_{k'}\rangle$ for $\forall d_i \in D$ will be compared, if they match, we insert the pair of target column and source column $\langle a_{k'}, a_{ik}\rangle$, into the hashmap that stores all mapping from target column to candidate columns.

Next, it searches for a minimal subset of raw datasets $D' \subset D$ so that for $\forall a_{k'} \in A^t$, $\exists d_i \in D$, satisfying that $\langle a_{k'}, a_{ik}\rangle$ exists in the hashmap.

Finally it performs join and filter operations over $D'$ to create and output the outcome integrated table. 

\noindent
\textbf{Analysis.} For the baseline algorithm, the computational overhead is mainly incurred by generating LSH signatures for all columns in the raw datasets, of which the complexity is $O((p+\sum_0^m{p_i})\times L)$, which can be carried out in offline style. The online overhead mainly includes the matching of all raw columns to each of the target columns, of which the complexity is $O(p\times \sum_0^m {p_i})$. 

In case of schema evolution and data updates, it requires to generate and store LSH signatures for each updated/newly-added column. This could be a prohibitive overhead for fast-evolving data sources.

In addition, the baseline algorithm also requires to store $(p+\sum_0^m{p_i})\times L$ signatures, which could be quite significant if the raw datasets are dominated by wide tables. 

Moreover, because the baseline algorithm is constrained by the simplifying assumptions that we mentioned earlier, it cannot be easily extended to semistructured and unstructured raw datasets, and raw datasets that spread target feature values as column/attribute names, as illustrated in Fig.~\ref{fig:schema-example}.




\subsection{An End-to-End Deep Learning Approach}
To provide a more flexible and efficient solution to handle integration of heterogeneous and fast evloving data, we further propose a novel approach based on deep learning.

\noindent
\textbf{1. Word Embedding.} 

\noindent
\textbf{2. Feature Representation.} For each raw dataset $d_i \in D = \{c_{ij}\}$, a data item is modeled as a key-value pair $ c_{ij} = \langle \vec{key}^{\vec{T}_{key_{ij}}}_{ij}, value^{T_{value_{ij}}}_{ij}\rangle $. Therefore, it is easy to store each raw dataset as a set of quadruples, in the form of (\texttt{key\_array}, \texttt{key\_type\_array}, \texttt{value}, \texttt{value\_type}) as illustrated in Fig.~\ref{fig:schema-example}. Each field in the quadruple is encoded based on a dictionary and can be decoded based on the type information. This transformation process that parses raw data into key-value representation is conducted offline at storage time. We will describe a few techniques to accelerate this process, such as data scheduling and sampling.

\noindent
\textbf{3. Label Representation.} On the other hand, the label to predict is formulated as a  $($\texttt{row\_key(s)}, \texttt{column\_attribute}, \texttt{aggregation\_mode}$)$ tuple that specifies the position $(a_k, r_l), a_k \in A^t, r_l \in R^t$ in the outcome table $V^{A^t \times R^t}$ as well as how values assigned to the same cell in the output table should be aggregated. We support multiple aggregation modes, such as arithmetic addition (\texttt{+}), string concatenation (\texttt{concat}), replace of the old value using the new value (\texttt{replace}), keep the old value and discard the new value (\texttt{discard}), and so on. The labeling process is illustrated in Fig.~\ref{fig:prediction}. In our implementation and experiments for this work, the label is represented as a one-hot vector.

\begin{figure}[h]
\centering
   \includegraphics[width=3.4in]{prediction.pdf}
\caption{\label{fig:prediction}
Illustration of the labeling process for the schema evolution with key expansions}
\end{figure}

\noindent
\textbf{4. Model Architecture.} We propose a three-layer neural network model architecture to learn the function (i.e. $f^{C\rightarrow (A^{t}\cup\{NULL\})\times (R^{t}\cup\{NULL\})}_t$) that maps the input feature quadruple ($c_{ij} \in d_i,\forall d_i \in D$) to its position in the outcome table ($(a_k, r_l), a_k \in A^t, r_l \in R^t$). The first layer is a word embedding layer. As advocated in DeepMatcher~\cite{mudgal2018deep}, using an existing character embedding trained with large corpus like Wikipedia data may improve the accuracy. We will consider such approach in our future works, and the last layer is a fully connected layer. For the middle layers, we try both RNN (LSTM) and CNN, and find that due to the locality (i.e. key array is irrelevant with value) is critical, CNN can achieve better accuracy.  We find that CNN performs better than LSTM in our preliminary experiments (Sec.~\ref{sec:experiments}).

\noindent
\textbf{5. Training Data Preparation.} To train the data integration model, the user needs to create a set of labeled training samples. The candidate training datasets and their mappings to the target outcome table can be manually determined, or automatically determined by leveraging existing data discovery and schema matching approaches. But once these are determined, due to the mappings are usually a finite set of rules, the labeling process can be easily automated by developing a python script to transform the datasets into a series of key-value pairs and corresponding labels. In addition, we automatically inject schema changes into the training data by pivoting dimensions, expanding keys, changing attribute names and so on.  

\noindent
\textbf{6. Model Training Process.}
We observe that it only takes up to several seconds' time for training in commodity hardware with GPU, and the training process only needs to be performed once. Despite of the schema changes of most types, a trained model can be reused many times to integrate updated or new data sources. Therefore, if the application is relatively stable compared to the data sources, the training overhead gets well amortized over multiple integration processes.

\noindent
\textbf{7. Output Table Assembling.}
For each prediction, a data dispatcher is responsible to assemble a triple (\texttt{row\_id}, \texttt{column\_id},  \texttt{value}) from it to describe $(a_k, r_l, value^{T_{value_{ij}}}_{ij})$, buffer it in local, and dispatch the tuples to users' registered deep learning workers once the buffer is full. At each deep learning worker, a client of our system is responsible to receive tuples and assemble tuples into tensors. In addition, if user has registered a number of workers to form a distributed cluster, the output table will be partitioned in a way to guarantee load balance and ensure the independent identical distribution (i.e. iid) to avoid introducing bias. Finally, if user hasn't registered any deep learning workers, the data will be written to local. 

\noindent
\textbf{8. Transfer Learning.}


\noindent
\textbf{Analysis.} For the deep learning approach, the offline overhead includes the transformation and storage of all raw datasets into key-value pairs, as well as the training expense. The online overhead is mainly in model inference, which can be accelerated by advanced hardwares, like GPU, FPGA, and ASIC.

The overall storage overhead is mainly caused by the storage of pre-trained models, which is linear to the number of different applications. However we find that the storage overhead for a single model is merely up to several to tens of kilobytes. One thing to note is that the proposed key-value model can also significantly reduce intermediate processing overhead for sparse data. In the future, we may consider to cache the key-value representation for reuse.

Once a data integration model is trained, there is almost no need for human intervention, despite of newly added or updated data sources, which also distinguishes it from the baseline approach and other existing works.

Finally the performance of the deep learning approach can be further optimized by using an early stopping mechanism. Instead of parsing all data items in the source datasets, we can parse only $n_k$ sampled items for each column, and we will skip the parsing of the rest of the column for testing if most of the sampled items are discarded. $n_k$ is determined by the number of values in the column.


\eat{
\subsection{Performance Optimization Techniques}
\label{sec:optimization}
The performance of the proposed deep learning approach can be further improved by applying an array of techniques. 
\subsubsection{Early Stopping} Instead of parsing all of the raw datasets and sending each key-value-based data item to the data integration model for labeling its position and aggregation mode in the outcome table, we can introduce an early stopping mechanism so that if a raw column's first $n_k$ items are discarded, we will skip this column and will not pass more data items from the column for testing. $n_k$ is determined by the number of values in the column.

\noindent
\textbf{Caching} In our proposed system, heterogeneous types of data are competing for memory resources, including the raw data repository, the pre-trained models, the outcome tables, and the history of user requests. We manage all data using the concept of locality sets that we propose in Pangea~\cite{zou2019pangea}. So that  data share similar locality patterns are grouped into the same locality set. Each locality set is labeled with its data location, access patterns, access recency and frequency, persistence requirements, preferred caching strategy and so on. A global scheduler will decide on the optimal caching strategy across all locality sets.

\noindent
\textbf{Parallelization} Concurrent data integration requests can be processed in parallel, so that the feature vector for one data item only needs to be cached once, but read by multiple models without additional fetching and memory-caching overhead.

\noindent
\textbf{Transfer Learning} If we cannot find an existing model with distance above a certain threshold to reuse for a new data integration request, we may use the closest model to initialize the parameters and perform a transfer learning to speedup the training process.
}
\eat{
\section{System Architecture}

\begin{figure} [h]
\centering
   \includegraphics[width=3.5in]{system-overview.pdf}
\caption{\label{fig:federated}
The automated data integration process}
\end{figure}

The proposed system is connected to heterogeneous data sources and consists of mainly seven components, as illustrated in Fig.~\ref{fig:federated}. 

\noindent
(1) \textbf{Data decomposition.} A dataset (e.g. text, JSON, CSV) needs to be decomposed into a stream of data items in the key-value representation for training and testing. 

\noindent
(2) \textbf{Training data generator.} This component will automatically convert user specified raw datasets into training samples and automatically inject schema evolutions and non-relevant data to ensure the diversity of training samples.

\noindent
(3) \textbf{Model library.} For each unique data integration request, we train a model that consists of an embedding layer, an LSTM layer, and a fully connected layer. Through the models,  a decomposed data item is mapped to its positions in the expected outcome tables by applying a certain aggregation mode of the data item's value and the original value in the target call if it exists or the data item is simply discarded. 

\noindent
(4) \textbf{Model selector.} Users need to specify the schema of expected outcome tables, as well as a few example rows for each table, as inputs. The system will match the expected table with the outcome tables of pre-trained models and find the most similar model to directly serve as the model or to simply initialize the new model parameters. 

\noindent
(5) \textbf{Storage manager.} All raw data, decomposed data items, output integrated data, pre-trained models, model traces are grouped into a few locality sets based on their access patterns~\cite{zou2019pangea}, and are all cached in memory. Whenever the working datasets exceed available memory, the storage manager will order all locality sets based on a cost model~\cite{zou2019pangea} and select a locality set to evict data from it.

\noindent
(6) \textbf{Data dispatcher.} The integrated data will be buffered and dispatched to remote deep learning workers that the user has registered with our system. Then at each deep learning worker's side, a client is running to assemble receoved key-value pairs into tensors so that the user's application can process it. The data dispatcher will guarantee load balance and feature/label distribution balance to avoid bias or skews.

\noindent
(7) \textbf{Trace sketcher.} This component will record mappings of each data item from its position in the source dataset to the predicted position in the target table. It will also summarize the distributions of mappings from source attributes to target attributes, in an attempt to explain the black box model.

{\color{red}{TODO: We need expand this high-level design, once we implement the key components.}}
}

==> problem.tex <==
\section{Problem Formulation}
\label{sec:problem}
In this section, we will first give an anatomy of main schema evolution types. Then we will formulate the problem.

\subsection{A Motivating Example}
\label{sec:example}
A data scientist wants to train a machine learning model to predict COVID-$19$ global outbreak. S/he needs features including date, country/region, subregion, population, confirmed COVID-$19$ cases, deaths, mobility to grocery, parks, restaurants, workplaces, and so on. Each time s/he may specify a range of dates and locations, and the row-keys (i.e. date, country/region/subregion) in the outcome table can be automatically populated correspondingly. Then the first question is that given two initially known and matching data sources, such as the daily updated Google mobility data~\cite{google-mobility} and JHU COVID-$19$ cases data~\cite{covid19-jhu}, of which the data is updated at daily basis and the schemas evolve at weekly basis, how to efficiently fill in the outcome table each time without much human intervention?  An extended and more interesting problem is that the users are given a large set of unknown data sources. Some data sources may be dead, which were once used for past data integration tasks, but is now outdated for new data integration requests. In the same time, new data sources are added dynamically. Then, how to automatically discover relevant data sources and fill in the user specified outcome table with minimum human manual efforts?

\eat{
Note that although most of raw datasets in the COVID-$19$ data repository are structured CSV files, they are not automatically joinable using an LSH-based approach~\cite{}. For example, a feature value could be embedded in the column names. For example, in the archived JHU time-series data ~\cite{}, each datetime is a column, and it has hundreds of columns for merely three months' data. Differently, in the Google mobility data, there is one column called datetime, and all time-series information are spreading into multiple rows other than columns. Such inconsistency significantly complicates the column matching problem. 

A manual approach requires to go through each column in each dataset and decide how data can be joined together to create the desired training samples. It takes a lot of efforts, particularly when there are a large number of candidate raw datasets.

In addition, we find that most of COVID-$19$ data updates at daily base, with multiple schema changes every month. Such frequent updates are not transparent to neither the LSH-based approach nor the manual approach, which requires additional overheads for updating LSH-signatures and/or the integration process.
}


\subsection{Data Model/Representation}


\subsection{Problem Definition}





